Slow Spin Relaxation and Low-Temperature Spin Freezing in Disordered Fluorite Ho$_2$Zr$_2$O$_7$

We report on the origin of spin freezing in the disordered fluorite Ho$_2$Zr$_2$O$_7$. The system is investigated by low-temperature heat capacity as well as by DC and AC magnetization. While the system does not show a long-range magnetic order down to at least $T = 280$~mK, we observe signatures of slow spin dynamics, magnetic field induced relaxation processes at relatively high temperatures, and a spin-frozen state below $T = 0.6$~K. Our results suggest that similar to the canonical spin ice systems Ho$_2$Ti$_2$O$_7$ [Ehlers 2004] and Dy$_2$Ti$_2$O$_7$ [Snyder 2001], spin freezing in Ho$_2$Zr$_2$O$_7$ is preceded by two slow spin relaxation processes; the first forms a field-induced region extending to at least 18~K and the second is rather field-independent and appears at $T_{\mathrm g2} = 1$~K [Ramon 2020].

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
